T-Cell Receptor Optimization with Reinforcement Learning and Mutation Policies for Precesion Immunotherapy

T cells monitor the health status of cells by identifying foreign peptides displayed on their surface. T-cell receptors (TCRs), which are protein complexes found on the surface of T cells, are able to bind to these peptides. This process is known as TCR recognition and constitutes a key step for immune response. Optimizing TCR sequences for TCR recognition represents a fundamental step towards the development of personalized treatments to trigger immune responses killing cancerous or virus-infected cells. In this paper, we formulated the search for these optimized TCRs as a reinforcement learning (RL) problem, and presented a framework TCRPPO with a mutation policy using proximal policy optimization. TCRPPO mutates TCRs into effective ones that can recognize given peptides. TCRPPO leverages a reward function that combines the likelihoods of mutated sequences being valid TCRs measured by a new scoring function based on deep autoencoders, with the probabilities of mutated sequences recognizing peptides from a peptide-TCR interaction predictor. We compared TCRPPO with multiple baseline methods and demonstrated that TCRPPO significantly outperforms all the baseline methods to generate positive binding and valid TCRs. These results demonstrate the potential of TCRPPO for both precision immunotherapy and peptide-recognizing TCR motif discovery.

==> tables/notations.tex <==
\begin{table}[!t]
  \centering
      \caption{Notations}
  \label{tbl:notations}
  \vspace{-10pt}

  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{0pt}}l@{\hspace{2pt}}
	@{\hspace{2pt}}p{0.8\linewidth}@{\hspace{2pt}}      
	}
        \toprule
        notation & meaning\\
        \midrule
        %\peptide     & peptide \\
        %\tcr         & TCR \\
        $\amino$/\tcr/\peptide   & amino acid/TCR sequence/peptide\\
        $\sta=(\tcr,\peptide)$   &  a state of environment\\
        $\action=(i,\amino)$  & an action of \RL agent ($i$: a mutation site, \amino: a mutant amino acid) \\
        $\reward$    & reward function \\
%        $\aminoemb$    & encoding of amino acid \\
%        $\hidden^{\peptide}$    & hidden vector of peptide in \tcrppo \\
%        $\hidden_{i,t}$    & hidden vector of $i$-th amino acid in $\tcr_t$ in \tcrppo \\
%        $\hidden_{t}$      & hidden vector of $\tcr_t$ in \tcrppo \\
%        $\hidden^\prime$    & hidden vector of a TCR in \autoenc \\
%        $\latent^{\prime}$      & latent vector of a TCR in \autoenc \\
%        \vTCRs/\bTCRs/\qTCRs             & set of valid/binding/qualified TCRs \\
%                     & set of binding TCRs \\
%        \qTCRs             & set of qualified TCRs \\
	\recog & probability of a TCR recognizing/binding to a peptide\\
%        \recog       & recognition probability for a TCR-peptide pair predicted by \ergo model.\\
%        $\sigma_r$   & threshold of recognition probability \\
        \istcr       & TCR validity score\\
%        $\sigma_c$   & threshold of \istcr to determine valid TCRs \\

        \bottomrule
      \end{tabular}
%      \begin{tablenotes}
%      \item 
%      \par
%      \end{tablenotes}
    \end{small}
  \end{threeparttable}
  \vspace{-15pt} 
\end{table}

==> tables/result_full.tex <==
\begin{table*}[!h]
	\centering
	\caption{Overall Performance Comparison}
	\label{tbl:perform:all}
	\begin{footnotesize}
		\begin{threeparttable}
			\begin{tabular}{
					%@{\hspace{5pt}}l@{\hspace{5pt}} % dataset
					%%
					@{\hspace{2pt}}l@{\hspace{2pt}} % method
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} % q
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} % edist
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}r@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} %stcr Q
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} % stcr V
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} % stcr b
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} % pr Q
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} % pr V
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} %pr B
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{2pt}}r@{\hspace{0pt}} % v
					@{\hspace{0pt}}c@{\hspace{0pt}}
					@{\hspace{0pt}}l@{\hspace{2pt}}
					%
					@{\hspace{0pt}}r@{\hspace{2pt}} % R
				}
				\toprule
                {Method} 
				& \multicolumn{3}{c}{{\qr}} 
				&  \multicolumn{3}{c}{{\mutediff}} 
				%
				& \multicolumn{3}{c}{\avgistcr(\qTCRs)}   & \multicolumn{3}{c}{\avgistcr(\vTCRs)} & \multicolumn{3}{c}{\avgistcr(\bTCRs)} 
				& \multicolumn{3}{c}{\avgrecog(\qTCRs)} & \multicolumn{3}{c}{\avgrecog(\vTCRs)} & \multicolumn{3}{c}{\avgrecog(\bTCRs)} 
				& \multicolumn{3}{c}{\vr}
				& \ncalls \\
				%
%				&  &  & & & & &&
%%				\multicolumn{3}{c}{\istcr>\istcrsigma $\land$ $\recog>\prsigma$} & \multicolumn{3}{c}{\{\istcr>\istcrsigma\}} & \multicolumn{3}{c}{$\recog>\prsigma$} & \multicolumn{3}{c}{\istcr>\istcrsigma $\land$ $\recog>\prsigma$} & \multicolumn{3}{c}{\{\istcr>\istcrsigma\}} & \multicolumn{3}{c}{$\recog>\prsigma$}  & \multicolumn{3}{c}{\vr} & \#\reward calls\\ 
%				\multicolumn{3}{c}{\vTCRs} & \multicolumn{3}{c}{\{\istcr>\istcrsigma\}} & \multicolumn{3}{c}{$\recog>\prsigma$} & \multicolumn{3}{c}{\istcr>\istcrsigma $\land$ $\recog>\prsigma$} & \multicolumn{3}{c}{\{\istcr>\istcrsigma\}} & \multicolumn{3}{c}{$\recog>\prsigma$}  & \multicolumn{3}{c}{\vr} & \#\reward calls\\ 
%			%	& &  1.51  &  $\pm$  &  0.07   &  1.42  &  $\pm$  &  0.10   &  1.53  &  $\pm$  &  0.08   &  0.83  &  $\pm$  &  0.09   &  0.94  &  $\pm$  &  0.02   &  0.93  &  $\pm$  &  0.02   &  76.29  &  $\pm$  &  8.22  &   &  39.84  &  $\pm$  &  27.61\\
				\midrule        
%<<<<<<< HEAD
%				& \randomselect   &  1.73  &  $\pm$  &  0.00   &  1.35  &  $\pm$  &  0.17   &  1.46  &  $\pm$  &  0.16   &  0.05  &  $\pm$  &  0.05   &  0.94  &  $\pm$  &  0.00   &  0.95  &  $\pm$  &  0.01   &  95.22  &  $\pm$  &  0.45   &  0.05  &  $\pm$  &  0.12   & & - & & 1 \\
%				\cmidrule{2-30}
%				\multirow{9}{*}{McPAS} 
%				& \mcts   &  1.34  &  $\pm$  &  0.03   &  1.38  &  $\pm$  &  0.00   &  1.38  &  $\pm$  &  0.00   &  0.09  &  $\pm$  &  0.09   &  0.93  &  $\pm$  &  0.00   &  0.93  &  $\pm$  &  0.00   &  0.59  &  $\pm$  &  0.28   &  0.01  &  $\pm$  &  0.03   & & - &  & 200\\
%				& \bpvae   &  1.34  &  $\pm$  &  0.02   &  1.28  &  $\pm$  &  0.04   &  1.31  &  $\pm$  &  0.02   &  0.09  &  $\pm$  &  0.04   &  0.94  &  $\pm$  &  0.01   &  0.95  &  $\pm$  &  0.02   &  6.86  &  $\pm$  &  2.52   &  0.04  &  $\pm$  &  0.09   & & - &  & 7.27\\
%=======
				%\multirow{9}{*}{\mcpasP}
				%&
				\multicolumn{29}{c}{{Dataset \mcpasP}}
				\\
				\cmidrule{1-29}
				\randomselect   &  0.05  &  $\pm$  &  0.12  
									&     &  -  &    
									&  1.46  &  $\pm$  &  0.16  
									&  1.73  &  $\pm$  &  0.17  
									&  1.35  &  $\pm$  &  0.00  
									&  0.95  &  $\pm$  &  0.01  
									&  0.05  &  $\pm$  &  0.00  
									&  0.94  &  $\pm$  &  0.05  
									&  95.22  &  $\pm$  &  0.45  
				& 1\\
				\cmidrule{1-29}						
				\mcts   &  0.01  &  $\pm$  &  0.03  
						   &    &  -  &    
							 &  1.38  &  $\pm$  &  0.00  
							&  1.34  &  $\pm$  &  0.03  
							&  1.38  &  $\pm$  &  0.00  
							&  0.93  &  $\pm$  &  0.00  
							&  0.09  &  $\pm$  &  0.09  
							&  0.93  &  $\pm$  &  0.00  
							&  0.59  &  $\pm$  &  0.28   
				& 200\\
			    \bpvae   &  0.04  &  $\pm$  &  0.09  
						   &     &  -  &    
							 &  1.31  &  $\pm$  &  0.02  
							&  1.34  &  $\pm$  &  0.02  
							&  1.28  &  $\pm$  &  0.04  
							&  0.95  &  $\pm$  &  0.02  
							&  0.09  &  $\pm$  &  0.04  
							&  0.94  &  $\pm$  &  0.01  
							&  6.86  &  $\pm$  &  2.52    
				& 7\\
				%
%>>>>>>> 23a72fc74a15c514b5246112dd2405639dbcc5f5
				\cmidrule{1-29}
				\randommutate (n=5)   &  1.27  &  $\pm$  &  2.09  
								&  2.88  &   $\pm$   & 1.50
								 &  1.49  &  $\pm$  &  0.07  
								&  1.54  &  $\pm$  &  0.02  
								&  1.49  &  $\pm$  &  0.07  
								&  0.93  &  $\pm$  &  0.02  
								&  0.18  &  $\pm$  &  0.09  
								&  0.93  &  $\pm$  &  0.02  
								&  99.36  &  $\pm$  &  0.21   
				& 39\\
				\randommutate (n=10)  &  2.15  &  $\pm$  &  3.86  
								&  3.04  &   $\pm$   & 1.48 
								 &  1.50  &  $\pm$  &  0.11  
								&  1.52  &  $\pm$  &  0.02  
								&  1.50  &  $\pm$  &  0.11  
								&  0.93  &  $\pm$  &  0.02  
								&  0.26  &  $\pm$  &  0.11  
								&  0.93  &  $\pm$  &  0.02  
								&  99.84  &  $\pm$  &  0.12   
				& 77\\
				\greedy   &  20.58  &  $\pm$  &  17.85  
								&  5.10   &  $\pm$  & 1.09
								 &  1.46  &  $\pm$  &  0.03  
								&  1.44  &  $\pm$  &  0.02  
								&  1.46  &  $\pm$  &  0.03  
								&  0.93  &  $\pm$  &  0.01  
								&  0.62  &  $\pm$  &  0.12  
								&  0.93  &  $\pm$  &  0.01  
								&  99.98  &  $\pm$  &  0.04   
				& 74\\
				\genetic   &  25.18  &  $\pm$  &  21.28  
								&  5.16  &  $\pm$  & 1.05
								 &  1.46  &  $\pm$  &  0.03  
								&  1.46  &  $\pm$  &  0.02  
								&  1.46  &  $\pm$  &  0.03  
								&  0.93  &  $\pm$  &  0.01  
								&  0.69  &  $\pm$  &  0.12  
								&  0.93  &  $\pm$  &  0.01  
								&  100.00  &  $\pm$  &  0.00 
				& 166\\
				\cmidrule{1-29}
%<<<<<<< HEAD
%				& \tcrppo   &  1.48  &  $\pm$  &  0.07   &  1.42  &  $\pm$  &  0.12   &  1.52  &  $\pm$  &  0.09   &  0.73  &  $\pm$  &  0.15   &  0.92  &  $\pm$  &  0.02   &  0.92  &  $\pm$  &  0.02   &  67.66  &  $\pm$  &  19.21   &  23.02  &  $\pm$  &  29.18   & 4.59  &   $\pm$   & 1.77 & 4.37\\
%				& \tcrppobuf   &  1.51  &  $\pm$  &  0.07   &  1.42  &  $\pm$  &  0.10   &  1.53  &  $\pm$  &  0.08   &  0.83  &  $\pm$  &  0.09   &  0.94  &  $\pm$  &  0.02   &  0.93  &  $\pm$  &  0.02   &  76.29  &  $\pm$  &  8.22   &  39.84  &  $\pm$  &  27.61   & 4.89  &   $\pm$   & 1.58 & 6.93\\
%%				   % & \tcrppo (+ buffer) & 77.60 & $\pm$ &  8.71 & 0.43 & $\pm$ & 0.34 & 0.96 & $\pm$ & 0.04 & 0.86 & $\pm$ & 0.08 & 0.56 & $\pm$ & 0.05 \\
%  	            	\midrule
% 				\multirow{9}{*}{VDJDB}
%				& \randomselect   &  1.73  &  $\pm$  &  0.01   &  1.44  &  $\pm$  &  0.28   &  1.58  &  $\pm$  &  0.20   &  0.03  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.02   &  95.02  &  $\pm$  &  0.46   &  0.08  &  $\pm$  &  0.10   & & - & & 1 \\
%				\cmidrule{2-30}
%				& \mcts   &  1.35  &  $\pm$  &  0.03   &  0.00  &  $\pm$  &  0.00   &  0.00  &  $\pm$  &  0.00   &  0.05  &  $\pm$  &  0.06   &  0.00  &  $\pm$  &  0.00   &  0.00  &  $\pm$  &  0.00   &  0.46  &  $\pm$  &  0.09   &  0.00  &  $\pm$  &  0.00   & & - &  & 200 \\
%				& \bpvae   &  1.35  &  $\pm$  &  0.01   &  1.27  &  $\pm$  &  0.04   &  1.33  &  $\pm$  &  0.03   &  0.05  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.01   &  0.95  &  $\pm$  &  0.03   &  18.46  &  $\pm$  &  5.13   &  0.08  &  $\pm$  &  0.12   & & - &  & 9.14\\
%%				& \randomselect   &  1.73  &  $\pm$  &  0.01   &  1.44  &  $\pm$  &  0.28   &  1.58  &  $\pm$  &  0.20   &  0.03  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.02   &  95.02  &  $\pm$  &  0.46   &  0.08  &  $\pm$  &  0.10   & & - & & 1 \\
%=======
				\tcrppo   &  23.02  &  $\pm$  &  29.18  
								&  4.59  &  $\pm$  & 1.77 
								  &  1.52  &  $\pm$  &  0.09  
								 &  1.48  &  $\pm$  &  0.07  
								 &  1.42  &  $\pm$  &  0.12  
								 &  0.92  &  $\pm$  &  0.02  
								 &  0.73  &  $\pm$  &  0.15  
								 &  0.92  &  $\pm$  &  0.02  
								 &  67.66  &  $\pm$  &  19.21  
				& 4\\
				\tcrppobuf   &  39.84  &  $\pm$  &  27.61  
								&  4.89  &  $\pm$  &  1.58
								  &  1.53  &  $\pm$  &  0.08  
								 &  1.51  &  $\pm$  &  0.07  
								 &  1.42  &  $\pm$  &  0.10  
								 &  0.93  &  $\pm$  &  0.02  
								 &  0.83  &  $\pm$  &  0.09  
								 &  0.94  &  $\pm$  &  0.02  
								 &  76.29  &  $\pm$  &  8.22 
				& 7\\
				\midrule
				%\multirow{9}{*}{\vdjdbP}
				%
				\multicolumn{29}{c}{{Dataset \vdjdbP}}
				\\
				\cmidrule{1-29}
				\randomselect   &  0.08  &  $\pm$  &  0.10  
								&     &  -  &    
								&  1.58  &  $\pm$  &  0.20  
								&  1.73  &  $\pm$  &  0.28  
								&  1.44  &  $\pm$  &  0.01  
								&  0.94  &  $\pm$  &  0.02  
								&  0.03  &  $\pm$  &  0.03  
								&  0.94  &  $\pm$  &  0.03  
								&  95.02  &  $\pm$  &  0.46  
				& 1\\
				\cmidrule{1-29}				
				\mcts   &  0.00  &  $\pm$  &  0.00  
								&     &  -  &     
								 &  0.00  &  $\pm$  &  0.00  
								&  1.35  &  $\pm$  &  0.03  
								&  0.00  &  $\pm$  &  0.00  
								&  0.00  &  $\pm$  &  0.00  
								&  0.05  &  $\pm$  &  0.06  
								&  0.00  &  $\pm$  &  0.00  
								&  0.46  &  $\pm$  &  0.09
				& 200\\
				\bpvae   &  0.08  &  $\pm$  &  0.12  
								&    &  -  &     
								  &  1.33  &  $\pm$  &  0.03  
								 &  1.35  &  $\pm$  &  0.01  
								 &  1.27  &  $\pm$  &  0.04  
								 &  0.95  &  $\pm$  &  0.03  
								 &  0.05  &  $\pm$  &  0.03  
								 &  0.94  &  $\pm$  &  0.01  
								 &  18.46  &  $\pm$  &  5.13  
				& 9\\
				%
%>>>>>>> 23a72fc74a15c514b5246112dd2405639dbcc5f5
				\cmidrule{1-29}
				\randommutate (n=5)  &  2.15  &  $\pm$  &  1.82  
								&  2.84  &  $\pm$  & 1.47  
								  &  1.48  &  $\pm$  &  0.09  
								 &  1.55  &  $\pm$  &  0.01  
								 &  1.48  &  $\pm$  &  0.09  
								 &  0.94  &  $\pm$  &  0.02  
								 &  0.16  &  $\pm$  &  0.06  
								 &  0.94  &  $\pm$  &  0.02  
								 &  99.33  &  $\pm$  &  0.21  
				& 39\\
				\randommutate (n=10)  &  4.41  &  $\pm$  &  3.72  
								&  3.03  &  $\pm$  & 1.52
								 &  1.48  &  $\pm$  &  0.07  
								&  1.52  &  $\pm$  &  0.02  
								&  1.48  &  $\pm$  &  0.07  
								&  0.94  &  $\pm$  &  0.01  
								&  0.24  &  $\pm$  &  0.08  
								&  0.94  &  $\pm$  &  0.01  
								&  99.86  &  $\pm$  &  0.08    
				& 77\\
				\greedy   &  31.81  &  $\pm$  &  17.09  
								&  5.01  &  $\pm$  & 1.12 
								 &  1.47  &  $\pm$  &  0.03  
								&  1.44  &  $\pm$  &  0.02  
								&  1.47  &  $\pm$  &  0.03  
								&  0.93  &  $\pm$  &  0.01  
								&  0.64  &  $\pm$  &  0.09  
								&  0.93  &  $\pm$  &  0.01  
								&  99.96  &  $\pm$  &  0.06   
				& 71\\
				\genetic   &  38.57  &  $\pm$  &  20.57  
								&  5.07  &  $\pm$  & 1.07
								 &  1.48  &  $\pm$  &  0.03  
								&  1.47  &  $\pm$  &  0.02  
								&  1.48  &  $\pm$  &  0.03  
								&  0.94  &  $\pm$  &  0.01  
								&  0.72  &  $\pm$  &  0.09  
								&  0.94  &  $\pm$  &  0.01  
								&  100.00  &  $\pm$  &  0.00  
				& 156\\
				\cmidrule{1-29}
				\tcrppo   &  48.90  &  $\pm$  &  25.13  
								&  4.62  &  $\pm$  & 1.53 
								 &  1.50  &  $\pm$  &  0.08  
								&  1.49  &  $\pm$  &  0.07  
								&  1.40  &  $\pm$  &  0.12  
								&  0.94  &  $\pm$  &  0.01  
								&  0.83  &  $\pm$  &  0.15  
								&  0.94  &  $\pm$  &  0.02  
								&  71.90  &  $\pm$  &  10.14 
				& 6\\
				\tcrppobuf   &  48.18  &  $\pm$  &  20.55  
								&  4.74  &  $\pm$  & 1.65 
							  &  1.52  &  $\pm$  &  0.10  
							 &  1.51  &  $\pm$  &  0.07  
							 &  1.41  &  $\pm$  &  0.15  
							 &  0.94  &  $\pm$  &  0.01  
							 &  0.83  &  $\pm$  &  0.15  
							 &  0.94  &  $\pm$  &  0.01  
							 &  72.50  &  $\pm$  &  9.68    
				& 6\\
%				& \mcts   &  1.34  &  $\pm$  &  0.03   &  1.38  &  $\pm$  &  0.00   &  1.38  &  $\pm$  &  0.00   &  0.09  &  $\pm$  &  0.09   &  0.93  &  $\pm$  &  0.00   &  0.93  &  $\pm$  &  0.00   &  0.59  &  $\pm$  &  0.28   &  0.01  &  $\pm$  &  0.03   & & - &  & 200\\
%				& \bpvae   &  1.34  &  $\pm$  &  0.02   &  1.28  &  $\pm$  &  0.04   &  1.31  &  $\pm$  &  0.02   &  0.09  &  $\pm$  &  0.04   &  0.94  &  $\pm$  &  0.01   &  0.95  &  $\pm$  &  0.02   &  6.86  &  $\pm$  &  2.52   &  0.04  &  $\pm$  &  0.09   & & - &  & 7.27\\
%				& \randomselect   &  1.73  &  $\pm$  &  0.00   &  1.35  &  $\pm$  &  0.17   &  1.46  &  $\pm$  &  0.16   &  0.05  &  $\pm$  &  0.05   &  0.94  &  $\pm$  &  0.00   &  0.95  &  $\pm$  &  0.01   &  95.22  &  $\pm$  &  0.45   &  0.05  &  $\pm$  &  0.12   & & - & & 1 \\
%				\cmidrule{2-30}
%				& \randommutate   &  1.54  &  $\pm$  &  0.02   &  1.49  &  $\pm$  &  0.07   &  1.49  &  $\pm$  &  0.07   &  0.18  &  $\pm$  &  0.09   &  0.93  &  $\pm$  &  0.02   &  0.93  &  $\pm$  &  0.02   &  99.36  &  $\pm$  &  0.21   &  1.27  &  $\pm$  &  2.09   & 2.88  &   $\pm$   & 1.50 & 39.34 \\
%				& \randommutate   &  1.52  &  $\pm$  &  0.02   &  1.50  &  $\pm$  &  0.11   &  1.50  &  $\pm$  &  0.11   &  0.26  &  $\pm$  &  0.11   &  0.93  &  $\pm$  &  0.02   &  0.93  &  $\pm$  &  0.02   &  99.84  &  $\pm$  &  0.12   &  2.15  &  $\pm$  &  3.86   & 3.04  &   $\pm$   & 1.48 & 77.53\\
%				& \greedy   &  1.44  &  $\pm$  &  0.02   &  1.46  &  $\pm$  &  0.03   &  1.46  &  $\pm$  &  0.03   &  0.62  &  $\pm$  &  0.12   &  0.93  &  $\pm$  &  0.01   &  0.93  &  $\pm$  &  0.01   &  99.98  &  $\pm$  &  0.04   &  20.58  &  $\pm$  &  17.85   & 5.10  &   $\pm$   & 1.09 &  74.39\\
%				& \genetic   &  1.46  &  $\pm$  &  0.02   &  1.46  &  $\pm$  &  0.03   &  1.46  &  $\pm$  &  0.03   &  0.69  &  $\pm$  &  0.12   &  0.93  &  $\pm$  &  0.01   &  0.93  &  $\pm$  &  0.01   &  100.00  &  $\pm$  &  0.00   &  25.18  &  $\pm$  &  21.28   & 5.16  &   $\pm$   & 1.05 &  165.81 \\
%				\cmidrule{2-30}
%				& \tcrppo   &  1.48  &  $\pm$  &  0.07   &  1.42  &  $\pm$  &  0.12   &  1.52  &  $\pm$  &  0.09   &  0.73  &  $\pm$  &  0.15   &  0.92  &  $\pm$  &  0.02   &  0.92  &  $\pm$  &  0.02   &  67.66  &  $\pm$  &  19.21   &  23.02  &  $\pm$  &  29.18   & 4.59  &   $\pm$   & 1.77 & 4.37\\
%				& \tcrppobuf   &  1.51  &  $\pm$  &  0.07   &  1.42  &  $\pm$  &  0.10   &  1.53  &  $\pm$  &  0.08   &  0.83  &  $\pm$  &  0.09   &  0.94  &  $\pm$  &  0.02   &  0.93  &  $\pm$  &  0.02   &  76.29  &  $\pm$  &  8.22   &  39.84  &  $\pm$  &  27.61   & 4.89  &   $\pm$   & 1.58 & 6.93\\
%%				   % & \tcrppo (+ buffer) & 77.60 & $\pm$ &  8.71 & 0.43 & $\pm$ & 0.34 & 0.96 & $\pm$ & 0.04 & 0.86 & $\pm$ & 0.08 & 0.56 & $\pm$ & 0.05 \\
%  	            	\midrule
% 				\multirow{9}{*}{VDJDB}
%				& \mcts   &  1.35  &  $\pm$  &  0.03   &  0.00  &  $\pm$  &  0.00   &  0.00  &  $\pm$  &  0.00   &  0.05  &  $\pm$  &  0.06   &  0.00  &  $\pm$  &  0.00   &  0.00  &  $\pm$  &  0.00   &  0.46  &  $\pm$  &  0.09   &  0.00  &  $\pm$  &  0.00   & & - &  & 200 \\
%				& \bpvae   &  1.35  &  $\pm$  &  0.01   &  1.27  &  $\pm$  &  0.04   &  1.33  &  $\pm$  &  0.03   &  0.05  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.01   &  0.95  &  $\pm$  &  0.03   &  18.46  &  $\pm$  &  5.13   &  0.08  &  $\pm$  &  0.12   & & - &  & 9.14\\
%				& \randomselect   &  1.73  &  $\pm$  &  0.01   &  1.44  &  $\pm$  &  0.28   &  1.58  &  $\pm$  &  0.20   &  0.03  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.03   &  0.94  &  $\pm$  &  0.02   &  95.02  &  $\pm$  &  0.46   &  0.08  &  $\pm$  &  0.10   & & - & & 1 \\
%				\cmidrule{2-30}
%				& \randommutate   &  1.55  &  $\pm$  &  0.01   &  1.48  &  $\pm$  &  0.09   &  1.48  &  $\pm$  &  0.09   &  0.16  &  $\pm$  &  0.06   &  0.94  &  $\pm$  &  0.02   &  0.94  &  $\pm$  &  0.02   &  99.33  &  $\pm$  &  0.21   &  2.15  &  $\pm$  &  1.82   & 2.84  &   $\pm$   & 1.47 & 39.31 \\
%				& \randommutate   &  1.52  &  $\pm$  &  0.02   &  1.48  &  $\pm$  &  0.07   &  1.48  &  $\pm$  &  0.07   &  0.24  &  $\pm$  &  0.08   &  0.94  &  $\pm$  &  0.01   &  0.94  &  $\pm$  &  0.01   &  99.86  &  $\pm$  &  0.08   &  4.41  &  $\pm$  &  3.72   & 3.03  &   $\pm$   & 1.52 &  77.05\\
%				& \greedy   &  1.44  &  $\pm$  &  0.02   &  1.47  &  $\pm$  &  0.03   &  1.47  &  $\pm$  &  0.03   &  0.64  &  $\pm$  &  0.09   &  0.93  &  $\pm$  &  0.01   &  0.93  &  $\pm$  &  0.01   &  99.96  &  $\pm$  &  0.06   &  31.81  &  $\pm$  &  17.09   & 5.01  &   $\pm$   & 1.12 &  70.77 \\
%				& \genetic   &  1.47  &  $\pm$  &  0.02   &  1.48  &  $\pm$  &  0.03   &  1.48  &  $\pm$  &  0.03   &  0.72  &  $\pm$  &  0.09   &  0.94  &  $\pm$  &  0.01   &  0.94  &  $\pm$  &  0.01   &  100.00  &  $\pm$  &  0.00   &  38.57  &  $\pm$  &  20.57   & 5.07  &   $\pm$   & 1.07 &  156.07 \\
%				\cmidrule{2-30}
%				& \tcrppo   &  1.49  &  $\pm$  &  0.07   &  1.40  &  $\pm$  &  0.12   &  1.50  &  $\pm$  &  0.08   &  0.83  &  $\pm$  &  0.15   &  0.94  &  $\pm$  &  0.02   &  0.94  &  $\pm$  &  0.01   &  71.90  &  $\pm$  &  10.14   &  48.90  &  $\pm$  &  25.13   & 4.62  &   $\pm$   & 1.53 & 6.06\\
%				& \tcrppobuf   &  1.51  &  $\pm$  &  0.07   &  1.41  &  $\pm$  &  0.15   &  1.52  &  $\pm$  &  0.10   &  0.83  &  $\pm$  &  0.15   &  0.94  &  $\pm$  &  0.01   &  0.94  &  $\pm$  &  0.01   &  72.50  &  $\pm$  &  9.68   &  48.18  &  $\pm$  &  20.55   & 4.74  &   $\pm$   & 1.65 &  6.13\\
				\bottomrule
			\end{tabular}
			\begin{tablenotes}
			%\begin{scriptnotesize}
			\item Columns represent: \qr: the percentage of qualified TCR sequences; 
			        \mutediff:  the edit distance between the original TCR sequences and the mutated qualified TCR sequences; 
			        $\avgistcr(\qTCRs)$/$\avgistcr(\vTCRs)$/$\avgistcr(\bTCRs)$: the average \istcr scores over the TCRs in set \qTCRs/\vTCRs/\bTCRs; %with all the generated qualified TCR sequences ($\{\istcr>\istcrsigma \land \recog>\prsigma\}$)/valid TCR sequences($\{\istcr>\istcrsigma\}$)/binding sequences($\{\recog>\prsigma\}$).
			        $\avgrecog(\qTCRs)$/$\avgrecog(\vTCRs)$/$\avgrecog(\bTCRs)$: the average \recog probabilities over the TCRs in set \qTCRs/\vTCRs/\bTCRs; % with all the generated qualified TCR sequences/valid TCR sequences/binding sequences.
			        \vr: the percentage of valid TCR sequences.
			        \ncalls: the average number of calls to calculate \reward functions. 
				Values $x\pm y$ represent mean $x$ and standard deviation $y$. 
			        ``-'': not applicable.
			        The ``$n$" value in \randommutate indicates that \randommutate is done $n$ times over each sequence. \par
			%\end{scriptnotesize}
			\end{tablenotes}
		\end{threeparttable}
	\end{footnotesize}
	%!TEX encoding = UTF-8 Unicode}
	\vspace{-10pt}    
\end{table*}

==> tables/statistics.tex <==
\begin{table}[!t]
  \centering
  \caption{{Data Statistics}}
  \label{tbl:stat}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{2pt}}l@{\hspace{2pt}}    	
	@{\hspace{2pt}}r@{\hspace{2pt}}    
	@{\hspace{5pt}}p{0.5\linewidth}@{\hspace{2pt}}    
	}
        \toprule
        Notation & Statistics & Used for\\
        \midrule
         \mcpasP & 10  &   peptides in \mcpas that TCRs are optimized to bind to\\
	%        
        \vdjdbP &15 &   peptides in \vdjdb that TCRs are optimized to bind to\\
        %
        \Train     & 7,281,064 &   TCRs from \tcrdb to train \tcrppo and \autoenc\\
        %
        \Validation &  50,000   &  valid TCRs from \tcrdb to validate \istcr scores,\\
        %
         \Test     & 1,000     &  initial TCRs to test \tcrppo, extracted from \Validation \\
        \bottomrule
      \end{tabular}
    \end{small}
  \end{threeparttable}
  \vspace{-13pt} 
\end{table}
